nomp: A Framework for Building Domain Specific Compilers

The low-level GPU programming models (CUDA, HIP, OpenCL, etc.) provide detailed control of the data flow and execution plan of a program in order to extract close-to-metal performance. However, these have a steep learning curve due to the intricacies of their syntax and semantics. This reduces programmer productivity. On the other hand, high-level models (OpenMP, OpenACC, etc.) that serve as abstractions over the low-level models are aimed at improving programmer productivity but achieving performance on-par with the low-level models is a challenge. There are inherent trade-offs between productivity, portability and performance in both approaches and there is no one-size-fits-all solution which achieves all three simultaneously. However, we believe there is room to improve programmer productivity without sacrificing performance and portability by reusing optimization patterns specific to a given domain. To this end, we propose nomp: a framework for building domain specific compilers. nomp consists of a pragma based programming model and a runtime capable of code transformation and generation based on user provided metadata.

==> tex/authors.tex <==
\author{Thilina Ratnayaka\affilnum{1,5}, Kaushik Kulkarni\affilnum{1,6},
Nipuna Fernando\affilnum{2}, Pubudu Hewavitharana\affilnum{2},
Hirumal Priyashan\affilnum{2}, Poorna Gunathilaka\affilnum{2},
Nagitha Abeywickrema\affilnum{2}, Ravindu Hirimuthugoda\affilnum{2},
Tarun Prabhu\affilnum{3}, Kirshanthan Sundararajah\affilnum{4}, and
Sanath Jayasena\affilnum{2}}

\affiliation{
\affilnum{1}Department of Computer Science, University of Illinois,
Urbana, IL 61801\\
\affilnum{2}Department of Computer Science, University of Moratuwa,
Katubedda 10400\\
\affilnum{3}Los Alamos National Laboratory, Los Alamos, NM 87545\\
\affilnum{4}Department of Computer Science, Virginia Tech, Blacksburg,
VA 24061\\
\affilnum{5}Argonne National Laboratory, Lemont, IL 60439\\
\affilnum{6}Qualcomm Research, San Diego, CA}

\corrauth{Thilina Ratnayaka, Department of Computer Science,
University of Illinois, IL 61801}
\email{tratnayaka@anl.gov}

